Solitary waves and double layers in complex plasma media

A complex plasma medium (containing Cairns nonthermal electron species, adiabatically warm inertial ion species, and stationary positively charged dust (PCD) species (making a plasma system very complex) is considered. The effects of PCD species, nonthermal electron species, and adiabatic ion-temperature on ion-acoustic (IA) solitary waves (SWs) and double layers (DLs) are investigated by the pseudo-potential approach, which is valid for the arbitrary amplitude time-independent SWs and DLs. It is observed that the presence of the PCD species reduces the phase speed of the IA waves, and consequently supports the IA subsonic compressive SWs in such electron-ion-PCD plasmas. On the other hand, the increase in both adiabatic ion-temperature and the number of nonthermal or fast electrons causes to reduce the possibility for the formation of the subsonic SWs, and thus convert subsonic SWs into supersonic ones. It is also observed that after at a certain value of the nonthermal parameter, the IA supersonic SWs with both positive and negative potentials as well as the DLs with only negative potential exist. The applications of the work in space environments (viz. Earth's mesosphere, cometary tails, Jupiter's magnetosphere, etc.) and laboratory devices, where the warm ion and nonthermal electron species along with PCD species have been observed, are briefly discussed.

==> biblo.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/

%% Created for A A Mamun at 2020-08-02 18:13:15 +0600


%% Saved with string encoding Unicode (UTF-8)


@preamble{"\providecommand{\noopsort}[1]{}" #
   "\providecommand{\singleletter}[1]{#1}%"}

@article{Havnes96,
	Author = {O. Havnes and J. Tr{\o}im and T. Blix and W. Mortensen and L. I. N{\ae}sheim and E. Thrane and T. T{\o}nnesen},
	Journal = {J. Geophys. Res.},
	Number = {A5},
	Pages = {10839},
	Title = {First detection of charged dust particles in the Earth's mesosphere},
	Volume = {101},
	Year = {1996}}
@article{Gelinas98,
	Author = {L. J. Gelinas and K. A. Lynch and M. C. Kelley and S. Collins and S. Baker and Q. Zhou and J. S. Friedman},
    Title = {First observation of meteoritic charged dust in the tropical mesosphere},
	Journal = {Geophys. Res. Lett.},
	Volume = {25},
    Number = {21},
	Pages = {4047-4050},
	Year = {1998}}
@article{Mendis04,
	Author = {D. A. Mendis and Wai-Ho Wong and M. Rosenberg},
    Title = {On the Observation of Charged Dust in the Tropical Mesosphere},
	Journal = {Phys. Scr.},
	Volume = {T113},
    Number = {},
	Pages = {141},
	Year = {2004}}
@article{Horanyi96,
	Author = {M. Hor\'anyi},
	Title = {Charged dust dynamics in the solar system},
    Journal = {Annu. Rev. Astron. Astrophys.},
    Volume = {34},
	Pages = {383},
	Year = {1996}}
@article{Mamun04,
	Author = {A. A. Mamun and P. K. Shukla},
    Title = {Dust-acoustic Mach cones in magnetized electron-dust plasmas of Saturn},
	Journal = {Geophys. Res. Lett.},
	Volume = {31},
    Number = {L06808},
	Pages = {1-4},
	Year = {2004}}
@article{Tsintikidis96,
	Author = {D. Tsintikidis and D. A. Gurnett and W. S. Kurth and L. J. Granroth},
    Title = {Micron-sized particles detected in the vicinity of Jupiter by the Voyager plasma wave instruments},
	Journal = {Geophys. Res. Lett.},
	Volume = {23},
    Number = {9},
	Pages = {997-1000},
	Year = {1996}}
@article{Horanyi93,
	Author = {M. Horanyi and G. E. Morfill and E. Gr\"un},
    Title = {Mechanism for the acceleration and ejection of dust grains from Jupiter's magnetosphere},
	Journal = {Nature},
	Volume = {363},
    Pages = {144-146},
	Year = {1993}}
@article{Khrapak01,
	Author = {S. A. Khrapak and G. Morfill},
    Title = {Waves in two component electron-dust plasma},
	Journal = {Phys. Plasmas},
	Volume = {8},
    Number = {6},
	Pages = {2629},
	Year = {2001}}
@article{Fortov03,
	Author = {V. E. Fortov and A. P. Nefedov and O. S. Vaulina and O. F. Petrov and I. E. Dranzhevski and A. M. Lipaev and Yu P. Semenov},
    Title = {Dynamics of dust grains in an electron–dust plasma induced by solar radiation under microgravity conditions},
	Journal = {New J. Phys.},
	Volume = {5},
    Number = {},
	Pages = {102.1–102.17},
	Year = {2003}}
@article{Davletov18,
	Author = {A. E. Davletov and F. Kurbanov and Ye. S. Mukhametkarimov},
    Title = {Chemical model for positively charged dust particles},
	Journal = {Phys. Plasmas},
	Volume = {25},
    Number = {12},
	Pages = {120701},
	Year = {2018}}
@article{Cairns95,
	Author = {R. A. Cairns and A. A. Mamun and R. Bingham and R. Bostr\"{o}m and R. O. Dendy and C. M. C. Nairn and P. K. Shukla},
	Journal = {Geophys. Res. Lett.},
	Title = {Electrostatic solitary structures in non‐thermal plasmas},
	Volume = {22},
    Number = {20},
	Pages = {2709},
	Year = {1995}}
@article{Chow93,
	Author = {V. W. Chow and D. A. Mendis and M. Rosenberg},
	Journal = {J. Geophys. Res.},
	Number = {A11},
	Pages = {19065},
	Title = {Role of grain size and particle velocity distribution in secondary electron emission in space plasmas},
	Volume = {98},
	Year = {1993}}
@article{Rosenberg95,
	Author = {M. Rosenberg and D. A. Mendis},
	Journal = {IEEE Trans. Plasma Sci.},
	Number = {2},
	Pages = {177},
	Title = {UV-induced Coulomb crystallization in a dusty gas},
	Volume = {23},
	Year = {1995}}
@article{Rosenberg96,
	Author = {M. Rosenberg and D. A. Mendis and D.P. Sheehan},
	Journal = {IEEE Trans. Plasma Sci.},
	Number = {6},
	Pages = {1422 - 1430},
	Title = {UV-induced Coulomb crystallization of dust grains in high-pressure gas},
	Volume = {24},
	Year = {1996}}
@article{Fortov98,
	Author = {V. E. Fortov and A. P. Nefedov and O. S. Vaulina and A. M. Lipaev and V. I. Molotkov and A. A. Samaryan and V. P. Nikitskii and A. I. Ivanov and S. F. Savin and A. V. Kalmykov and A. Ya. Solov'ev and P. V. Vinogradov},
	Journal = {JETP},
	Pages = {1087},
	Title = {Dusty plasma induced by solar radiation under microgravitational conditions: An experiment on board the Mir orbiting space station},
	Volume = {87},
	Year = {1998}}
@article{MS20,
	Author = {A. A. Mamun and B. E. Sharmin},
    Title = {Nonplanar ion-acoustic subsonic shock waves in dissipative electron-ion-pcd plasmas},
	Journal = {AIP Advances},
	Volume = {10},
    Number = {12},
	Pages = {125317},
	Year = {2020}}
@article{Mamun21,
	Author = {A. A. Mamun},
    Title = {Roles of positively charged dust in the formation of ion-acoustic subsonic solitary waves in electron-ion-pcd plasmas},
	Journal = {Contrib. Plasma Phys.},
	Volume = {61},
    Number = {1},
	Pages = {0},
	Year = {2021}}
@article{Mamun97,
	Author = {A. A. Mamun},
    Title = {Effects of ion temperature on electrostatic solitary structures in nonthermal plasmas},
	Journal = {Phys. Rev. E},
	Volume = {55},
    Number = {2},
	Pages = {1852},
	Year = {1997}}

@article{Bernstein57,
	Author = {I. B. Bernstein and G. M. Greene and M. D. Kruskal},
    Title = {Exact Nonlinear Plasma Oscillations},
	Journal = {Phys. Rev.},
	Volume = {108},
    Number = {3},
	Pages = {546},
	Year = {1957}}
@article{Nakamura2001,
	Author = {Y. Nakamura and A. Sarma},
    Title = {Observation of ion-acoustic solitary waves in a dusty plasma},
	Journal = {Phys. Plasmas},
	Volume = {8},
    Number = {9},
	Pages = {3921},
	Year = {2001}}
@article{Havnes01,
	Author = {O. Havnes and T. Aslaksen and A. Brattli},
    Title = {Charged dust in the Earth's middle atmosphere},
	Journal = {Phys. Scr.},
	Volume = {T89},
    Number = {},
	Pages = {133-137},
	Year = {2001}}
@article{Zedan20,
author = { N. A. Zedan and A. Atteya and W. F. El-Taibany and S. K. EL-Labany},
title = {Stability of ion-acoustic solitons in a multi-ion degenerate plasma with the effects of trapping and polarization under the influence of quantizing magnetic field},
journal = {Waves in Random and Complex Media},
volume = {0},
number = {0},
pages = {1-15},
year  = {2020}}
@article{El-Monier20,
author = {S. Y. El-Monier and A. Atteya},
title = {Dynamics of ion-acoustic waves in nonrelativistic magnetized multi-ion quantum plasma: the role of trapped electrons},
journal = {Waves in Random and Complex Media},
volume = {0},
number = {0},
pages = {1-19},
year  = {2020}}
@article{Mehdipoor20,
author = { M. Mehdipoor},
title = {Characteristics of nonlinear ion-acoustic waves in collisional plasmas with ionization effects},
journal = {Waves in Random and Complex Media},
volume = {0},
number = {0},
pages = {1-25},
year  = {2020}}
%@article{,
%	Author = {},
%    Title = {},
%	Journal = {},
%	Volume = {},
%    Number = {},
%	Pages = {},
%	Year = {}}

